Online Approval Committee Elections

Assume $k$ candidates need to be selected. The candidates appear over time. Each time one appears, it must be immediately selected or rejected -- a decision that is made by a group of individuals through voting. Assume the voters use approval ballots, i.e., for each candidate they only specify whether they consider it acceptable or not. This setting can be seen as a voting variant of choosing $k$ secretaries. Our contribution is twofold. (1) We assess to what extent the committees that are computed online can proportionally represent the voters. (2) If a prior probability over candidate approvals is available, we show how to compute committees with maximal expected score.

==> sections/old_related_work.tex <==
\section{Related work} \label{sec:related}

\paragraph{Online selection problems}
Our setting is close to generalized secretary problems \citep{babaioff2008online}, where the goal is to hire the best possible subset of candidates among a finite set of candidates arriving one at a time. A candidate's value is revealed upon arrival,
and the hiring decision must be taken immediately and cannot be changed afterwards. The connection between our work and this class of problems is detailed in Section \ref{sec:worstcase}. \citet{yu2019bi} consider a bi-criteria secretary problem with multiple choices, where each criterion can be seen as a voter, the subset of choices as the elected committee, and their objective function as the multiwinner approval voting objective. We consider instead a multiplicity of voters, and various objectives corresponding to Thiele rules in multiwinner voting. In the multi-attribute secretary problem \citep{bearden2005multi}, there are multiple independent attributes (e.g., skills), and the goal is to select the candidate that maximises the sum of payoffs on each of these attributes. This is equivalent to standard approval voting in our setting (for a committee of size 1). %candidates are ranked from best to worst on each of these attributes. The objective is the sum of payoffs for each of these attributes, and the goal is to select the single best candidate. This is equivalent to standard approval voting in our setting (for a committee of size 1).  
In the context of search engines, \cite{panigrahi2012online} directly aim to find an optimally diverse set of content from an input stream of items, by maximizing a coverage function for multiple features. In our committee election framework, items can be seen as candidates and features as voters, yet their objective function is different from the committee scoring functions we consider.
%\cite{stoyanovich2018online} also address the problem of hiring a team with candidates arriving online, but diversity constraints are enforced. In the context of search engines, \cite{panigrahi2012online} directly aim to find a maximally diverse set of content from input data streams. 

\paragraph{Social choice in online settings} Our work is mainly related to the study of proportional representation in committee (or multiwinner) elections, and in particular approval-based committee elections, which are surveyed in \citep{lac-sko:abc-survey}. In recent years, there has been increased interest in studying online versions of voting problems. Proportionality is studied in \citep{dey2017proportional} who formalize voting streams, a setting in which alternatives are fixed, but voters arrive in an online manner, which is the opposite to ours. In \citep{freeman2017fair}, the sets of voters and alternatives are fixed, but the valuations of each voter for an alternative varies over time. %At each timestep, one single alternative is chosen by a dynamic social choice function. 
Utilities are defined at each timestep as the cumulative reward of each agent given past decisions, and Nash social welfare is chosen to efficiently balance between fairness and efficiency. %The setting of ``perpetual voting'' from \cite{lackner2020perpetual} is similar but they consider ordinal preferences instead of cardinal valuations, which makes the definition of long-term effects more complex. 
\citet{lackner2020perpetual} consider a similar setting with ordinal preferences instead of cardinal valuations, which makes the definition of long-term effects more complex.
%They propose voting rules that weigh agents according to their satisfaction given past decisions, and how much other agents support their preferred alternative, in a way that favors agents that have been under-served in the past. %\cite{parkes2013dynamic} examine a similar problem to \cite{freeman2017fair}, by modeling agents’ evolving preferences with MDPs in which the reward depends on the chosen alternative, but they do not consider fairness. 
Other works address the partial observability of voters' preferences \citep{hossain2020designing}, or reweight voters over time based on a measure of the quality of their past votes \citep{haghtalab2018weighted}. 

While these works study (repeated) single-winner elections, the only existing work on online multiwinner elections to our knowledge is \citep{oren2014online}. The difference with our setting is that they consider online random arrival of voters rather than candidates, and they do not study proportionality axioms. \citet{do2021online} also study a close problem to ours, i.e. selecting a fixed size committee from an input stream of candidates based on irrevocable accept/reject decisions. A major difference is the absence of voters in their case. Proportionality is then defined based on multiple demographic attributes and a distance to target proportions on these attributes.

Recent studies address fairness in online versions of other social choice problems such as participatory budgeting \citep{lackner2021fairness} and proportional rankings \citep{israel2021dynamic}. There are also a number of works on online fair division, which we do not review as they are quite far from our concerns, because they deal with private domains.


% \virginie{ I shortened the description of these two for the sake of space:

% In \citep{haghtalab2018weighted}, the set of voters is fixed, and voters must vote for a different set of alternatives at each timestep. Across rounds, voters are re-weighted according to the quality of their past votes: a voter's ballot has more weight if they voted for good alternatives in the past. The authors design strategies inspired by no-regret learning.
% \cite{hossain2020fair} study a multi-agent version of the multi-armed bandit problem. Pulling an arm generates a stochastic reward for each agent, and the aim is to learn a fair distribution  over the arms, where fairness is measured by Nash social welfare.}


% \paragraph{Other online selection problems} 

% There are four different versions of the secretary problem, the articles we have cited before are from the first one, where the goal is to maximize the probability of getting the best secretary with no information. The Robbins' problem which is known as the fourth secretary problem is  explained in \cite{bruss_2005}. The goal is to maximize the expected rank of the alternative we select, with a knowledge of the probability distribution.  The diverse hiring setting of \cite{schumann2019diverse} is very different. At each time step, the decision-maker chooses which candidate to interview and only decides on which subset to hire after multiple rounds, whereas in our setting, candidates arrive one by one and decisions are made immediately.

==> sections/oldold_related_work.tex <==


Our work is mainly related to multiwinner elections. A good entry point in this literature is \citep{faliszewski2017multiwinner}.

\paragraph{Secretary problems} Generalized secretary problems \citep{babaioff2008online} are a class of 
optimal stopping problems where the goal is to hire the best possible subset of persons, assuming that persons arrive one at a time, their value is observed at that time,
and the decision to hire or not them must be taken immediately. The problem has been generalized to finding a set of items maximizing a submodular value function \citep{bateni2013submodular,badanidiyuru2014streaming}. 
%which can be applied to maximizing diversity. 
While the latter models do not deal with diversity constraints, %the recent work  
\cite{stoyanovich2018online} aims at selecting a group of people arriving in a streaming fashion from a finite pool, with the goal of optimizing their overall quality subject to diversity constraints. 

In the multi-attribute secretary problem \citep{bearden2005multi}, there are multiple attributes (e.g., skills), and candidates can be ranked from best to worst on each of these attributes, which are assumed independent. The objective is the sum of the payoffs for each of these attributes, and the goal is to select the single best candidate. This is equivalent to standard approval voting in our setting (for a committee of size 1).

Our setting with finite horizon and iid arrivals is the usual setting in online selection problems (e.g. Th. 2 in  \citep{panigrahi2012online}).

\paragraph{Social choice in online settings}

\cite{dey2017proportional} formalize voting streams, a setting in which alternatives are fixed, but voters arrive in an online manner. 

In \citep{freeman2017fair}, the sets of voters and alternatives are fixed, but the valuations of each voter for an alternative varies over time. At each timestep, one single alternative is chosen by a dynamic social choice function. Utilities are defined at each timestep as the cumulative reward of each agent given past decisions, and Nash social welfare is chosen to efficiently balance between fairness and efficiency.

The setting of ``perpetual voting'' from \cite{lackner2020perpetual} is similar but they consider ordinal preferences instead of cardinal valuations, which makes the definition of long-term effects more complex. They propose voting rules that weigh agents according to their satisfaction given past decisions, and how much other agents support their preferred alternative, in a way that favors agents that have been under-served in past decisions.

\cite{parkes2013dynamic} examine a similar problem to \cite{freeman2017fair}, by modeling agents’ evolving preferences with MDPs in which the reward depends on the chosen alternative, but they do not consider fairness.

In \citep{haghtalab2018weighted}, the set of voters are fixed, and voters must vote for a different set of alternatives at each timestep. Across rounds, voters are re-weighted according to the quality of their past votes: a voter's ballot has more weight if they voted for good alternatives in the past. The authors design strategies inspired by no-regret learning.

\cite{hossain2020fair} study a multi-agent version of the multi-armed bandit problem. Pulling an arm generates a stochastic reward for each agent, and the aim is to learn a fair distribution  over the arms, where fairness is measured by Nash social welfare.

There are also a number of works on online fair division, which we do not review as they are quite far from our concerns, because they deal with private domains.

\paragraph{Other online selection problems} 

There are four different versions of the secretary problem, the articles we have cited before are from the first one, where the goal is to maximize the probability of getting the best secretary with no information. The Robbins' problem which is known as the fourth secretary problem is  explained in \cite{bruss_2005}. The goal is to maximize the expected rank of the alternative we select, with a knowledge of the probability distribution.  The diverse hiring setting of \cite{schumann2019diverse} is very different. At each time step, the decision-maker chooses which candidate to interview and only decides on which subset to hire after multiple rounds, whereas in our setting, candidates arrive one by one and decisions are made immediately.

